Text-Derived Knowledge Helps Vision: A Simple Cross-modal Distillation for Video-based Action Anticipation

Anticipating future actions in a video is useful for many autonomous and assistive technologies. Most prior action anticipation work treat this as a vision modality problem, where the models learn the task information primarily from the video features in the action anticipation datasets. However, knowledge about action sequences can also be obtained from external textual data. In this work, we show how knowledge in pretrained language models can be adapted and distilled into vision-based action anticipation models. We show that a simple distillation technique can achieve effective knowledge transfer and provide consistent gains on a strong vision model (Anticipative Vision Transformer) for two action anticipation datasets (3.5% relative gain on EGTEA-GAZE+ and 7.2% relative gain on EPIC-KITCHEN 55), giving a new state-of-the-art result.

==> 3.4_ensembling.tex <==
\subsection{Ensembling Teacher Predictions}
With the recent progress in language modelling has led to the development of multiple pre-trained LMs which differ from one another on various factors such as training data, training loss, model architecture etc. 
Different pre-trained LMs exploits certain structure in the text that are complementary to one another. 
Consider a given training data $(\mathbf{X}, Y) \in \mathcal{D}, \mathbf{X} = [\mathbf{V}, \mathbf{S}]$ with $\mathbf{S}$ and $\mathbf{V}$ being the text and the vision modality features of the observed video $\mathbf{X}$ and $Y$ is the action label of the corresponding query segment $X_q$.
% 
Assume that we have $n$ different trained teachers and one student model that is trained using the predictions from the teacher as the label prior.
For a training data $(\mathbf{\{ S, V \}}, Y)$, the $i^{th}$, the teacher generates a set of feature and label $\{ f^*_{T_i}, \hat{Y}^*_{T_i}\}$, and the corresponding feature and label generated by the student model is given by $\{ f_{S}, \hat{Y}_{S}\}$.
The core idea of the proposed ensembling methodology is that the student should learn to focus on the teacher predictions based on the interaction between it's input representation and the corresponding representations generated by the teachers. This is done by using multi-headed cross-attention between the student and the teacher representation of the input.\\
For a $H$ headed adaptive ensembling, the ensembling coefficients for the teacher predictions for head $h$ and the overall coefficient is given by:
% 
\begin{align}
    & k_{i_h} = \mathbf{W_{kh}}\cdot f^*_{T_i} + \mathbf{b_{kh}} \nonumber \\
    & q_h = \mathbf{W_{qh}}\cdot f_{S} + \mathbf{b_{qh}} \nonumber \\
    & \alpha_{i_h} = \frac{\exp{(\langle k_{i_h}, q_{h} \rangle)}}{\sum_j \exp{(\langle k_{i_h}, q_{h} \rangle)}} \nonumber \\
    & \alpha_{i} = \sum^{H}_{h=1} \alpha_{i_h} \nonumber \\
    & \hat{Y}^*_{T_{ens}} = \sum_{i=1}^n{\alpha_i \cdot \hat{Y}^*_{T_i}} \nonumber
\end{align}
The ensembled teacher prediction $\hat{Y}^*_{T_{ens}}$ is then used as a label prior for the student for knowledge distillation.


==> 5.2_ablation.tex <==
\subsection{Ablation Analysis}

% --------------------------------------------------------------------------
% Factor 1
% --------------------------------------------------------------------------
\subsection{Effect of pre-training LM on domain relevant text on the teacher performance}: 
% 
\begin{table}[H]
\centering
\caption{Top-1 teacher accuracy of different datasets for different LM initialization}
\begin{tabular}{|p{0.16\linewidth} | p{0.21\linewidth} | p{0.1\linewidth} p{0.07\linewidth} p{0.07\linewidth} p{0.07\linewidth} p{0.09\linewidth}|}\hline
\multirow{2}{*}{Dataset}    & \multirow{2}{*}{LM initialization} & \multicolumn{5}{c|}{Teacher LM base}  \\ \cline{3-7}
                            &  & DistilBERT	& Electra	& Albert	& BERT	& RoBERTa  \\ \hline
\multirow{2}{*}{\texttt{EPIC-55}} & Standard Checkpoint & 18.33 & 11.88 & 14.70 & 19.12 & 17.79 \\ \cline{2-7}
                         & MLM on 1M Recipe & 19.10 & 17.09 & 17.73 & 18.53 & 18.47 \\ \hline
\multirow{2}{*}{\texttt{EGTEA GAZE+}} & Standard Checkpoint & 21.46 & 20.18 & 19.49 & 21.46 & 20.03 \\ \cline{2-7}
                         & MLM on 1M Recipe & 21.86	& 21.46	& 21.66	& 22.06	& 19.98 \\ \hline
\end{tabular}
\label{Table:ablation1}
\end{table}
% 
Here we analyse the effect of pre-training the teacher LM base on the teacher performance. 

% --------------------------------------------------------------------------
% Factor 2
% --------------------------------------------------------------------------
\subsection{Effect of Distillation loss on the task performance}: 
% 
\begin{table}[H]
\centering
\caption{Variation of model performance with distillation loss coefficient $\lambda_S$}
\begin{tabular}{|p{0.35\linewidth} | p{0.07\linewidth} | p{0.07\linewidth} | p{0.07\linewidth} | p{0.07\linewidth} | p{0.07\linewidth} |}\hline
$\mathbf{\lambda_S} $ & $\lambda_1$ & $\lambda_2$ & $\lambda_3$ & $\lambda_4$ & $\lambda_5$ \\ \hline
Top-1 accuracy & $-$ & $-$ & $-$ & $-$ & $-$ \\ \hline
Top-5 Many shot class mean recall & $-$ & $-$ & $-$ & $-$ & $-$ \\ \hline
\end{tabular}
\label{Table:ablation2}
\end{table}

% --------------------------------------------------------------------------
% Factor 3
% --------------------------------------------------------------------------
\subsection{Effect of number of heads on Ensembling performance}: 
\begin{table}[ht]
\centering
\caption{Variation of model performance with number of heads $H$ in the adaptive ensembling}
\begin{tabular}{|p{0.35\linewidth} | p{0.07\linewidth} | p{0.07\linewidth} | p{0.07\linewidth} | p{0.07\linewidth} | p{0.07\linewidth} |}\hline
$\mathbf{H} $ & $h_1$ & $h_2$ & $h_3$ & $h_4$ & $h_5$ \\ \hline
Top-1 accuracy & $-$ & $-$ & $-$ & $-$ & $-$ \\ \hline
Top-5 Many shot class mean recall & $-$ & $-$ & $-$ & $-$ & $-$ \\ \hline
\end{tabular}
\label{Table:ablation3}
\end{table}

% --------------------------------------------------------------------------
% Factor 4
% --------------------------------------------------------------------------
\subsection{Effect of aggregation strategy used for ensembling teacher predictions, on the model performance}: 
\begin{table}[ht]
\centering
\caption{Variation of model performance with the choice of teacher ensembling strategy}
\begin{tabular}{|p{0.35\linewidth} | p{0.15\linewidth} | p{0.19\linewidth} | p{0.17\linewidth} |}\hline
Ensebling strategy & Mean-pooling & Weighted average & Cross-attention \\ \hline
Top-1 accuracy & $-$ & $-$ & $-$  \\ \hline
Top-5 Many shot class mean recall & $-$ & $-$ & $-$ \\ \hline
\end{tabular}
\label{Table:ablation4}
\end{table}
